Bipartite Conditional Random Fields for Panoptic Segmentation

We tackle the panoptic segmentation problem with a conditional random field (CRF) model. Panoptic segmentation involves assigning a semantic label and an instance label to each pixel of a given image. At each pixel, the semantic label and the instance label should be compatible. Furthermore, a good panoptic segmentation should have a number of other desirable properties such as the spatial and color consistency of the labeling (similar looking neighboring pixels should have the same semantic label and the instance label). To tackle this problem, we propose a CRF model, named Bipartite CRF or BCRF, with two types of random variables for semantic and instance labels. In this formulation, various energies are defined within and across the two types of random variables to encourage a consistent panoptic segmentation. We propose a mean-field-based efficient inference algorithm for solving the CRF and empirically show its convergence properties. This algorithm is fully differentiable, and therefore, BCRF inference can be included as a trainable module in a deep network. In the experimental evaluation, we quantitatively and qualitatively show that the BCRF yields superior panoptic segmentation results in practice.

==> figs/pascal_all.tex <==
\begin{table*}[h!]
\vspace{-0.8cm}
%  \centering
	\begin{subtable}
        \centering
        {\renewcommand{\arraystretch}{0.7}
                                \begin{tabular}{ c@{\hspace{3pt}} c@{\hspace{3pt}} c@{\hspace{3pt}} c@{\hspace{3pt}} c}				
						\includegraphics[width=0.19\textwidth]{figs/pascal/original/144.jpg}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_sem/144.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_ins/144.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_sem/144.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_ins/144.png}\\
														\newline
						\includegraphics[width=0.19\textwidth]{figs/pascal/original/421.jpg}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_sem/421.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_ins/421.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_sem/421.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_ins/421.png}\\
						                                \newline
						\includegraphics[width=0.19\textwidth]{figs/pascal/original/438.jpg}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_sem/438.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_ins/438.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_sem/438.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_ins/438.png}\\
						                               \newline
						\includegraphics[width=0.19\textwidth]{figs/pascal/original/468.jpg}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_sem/468.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/before_ins/468.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_sem/468.png}%
						& \includegraphics[width=0.19\textwidth]{figs/pascal/after_ins/468.png}\\
														\newline
						\includegraphics[width=0.19\textwidth]{figs/pascal/original/184.jpg}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/before_sem/184.png}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/before_ins/184.png}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/after_sem/184.png}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/after_ins/184.png}\\
                                                        \newline
						\includegraphics[width=0.19\textwidth]{figs/pascal/original/226.jpg}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/before_sem/226.png}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/before_ins/226.png}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/after_sem/226.png}%
                        & \includegraphics[width=0.19\textwidth]{figs/pascal/after_ins/226.png}\\
%                                                          \newline
%  						\includegraphics[width=0.19\textwidth]{figs/pascal/original/233.jpg}%
%                          & \includegraphics[width=0.19\textwidth]{figs/pascal/before_sem/233.png}%
%                          & \includegraphics[width=0.19\textwidth]{figs/pascal/before_ins/233.png}%
%                          & \includegraphics[width=0.19\textwidth]{figs/pascal/after_sem/233.png}%
%                          &\includegraphics[width=0.19\textwidth]{figs/pascal/after_ins/233.png}\\														
% 														
                                \end{tabular}
                                }
    \end{subtable}
    \vspace{0.0cm}
    \caption{{\bf Visualizations on Pascal VOC.} Example images from the Pascal VOC validation set. Columns left to right: original image, semantic output before BCRF, instance output before BCRF, semantic output after BCRF, instance output after BCRF. Each row contains a new image. The standard Pascal VOC color map is used for the semantic segmentation results.}
    \label{tbl:pascal_visual}
    \vspace{-0.1cm}
\end{table*}


==> figs/tbl_pascal_detailed.tex <==
\begin{table*}[t]
	\vspace{-0.2cm}
	\hspace{0.2cm}
	\centering
	{\arraybackslash
\begin{tabular}{l|c|c|c|c|c|c}
	\hline
	\textbf{}	         & \multicolumn{2}{c|}{\textbf{PQ}} & \multicolumn{2}{c|}{\textbf{SQ}} & \multicolumn{2}{c}{\textbf{RQ}}  \\ \hline
	\textbf{Class}       & W/O BCRF       & BCRF            & W/O BCRF        & BCRF           & W/O BCRF        & BCRF           \\ \hline
	\textbf{Background}  & 90.8           & 92.33           & 93.39           & 94.69          & 97.22           & 97.51          \\ \hline
	\textbf{Aeroplane}   & 78.55          & 80.37           & 88.57           & 92.6           & 88.68           & 86.79          \\ \hline
	\textbf{Bicycle}     & 29.78          & 31.71           & 67.36           & 68.46          & 44.21           & 46.32          \\ \hline
	\textbf{Bird}        & 84.98          & 85.09           & 93.05           & 93.24          & 91.32           & 91.25          \\ \hline
	\textbf{Boat}        & 65.83          & 66.21           & 85.33           & 86.48          & 77.14           & 76.56          \\ \hline
	\textbf{Bottle}      & 67.44          & 64.05           & 92.05           & 90.68          & 73.26           & 70.63          \\ \hline
	\textbf{Bus}         & 82.68          & 82.58           & 94.56           & 95.46          & 87.44           & 86.51          \\ \hline
	\textbf{Car}         & 72.22          & 70.93           & 93.69           & 91.7           & 77.08           & 77.35          \\ \hline
	\textbf{Cat}         & 77.41          & 83.4            & 91.24           & 93.73          & 84.85           & 88.97          \\ \hline
	\textbf{Chair}       & 43.3           & 41.79           & 82.5            & 82.64          & 52.49           & 50.57          \\ \hline
	\textbf{Cow}         & 76.91          & 80.42           & 92.81           & 93.95          & 82.87           & 85.6           \\ \hline
	\textbf{Diningtable} & 51.33          & 51.8            & 80.81           & 82.88          & 63.51           & 62.5           \\ \hline
	\textbf{Dog}         & 76.63          & 81.59           & 90.5            & 93.29          & 84.67           & 87.46          \\ \hline
	\textbf{Horse}       & 76.86          & 81.4            & 89.38           & 91.11          & 86              & 89.34          \\ \hline
	\textbf{Motorbike}   & 78.07          & 80.21           & 87.5            & 89.89          & 89.23           & 89.23          \\ \hline
	\textbf{Person}      & 76.33          & 77              & 89.75           & 89.73          & 85.05           & 85.81          \\ \hline
	\textbf{Pottedplant} & 58.98          & 60.62           & 85.41           & 85.32          & 69.06           & 71.05          \\ \hline
	\textbf{Sheep}       & 74.29          & 74              & 93.86           & 93.48          & 79.15           & 79.15          \\ \hline
	\textbf{Sofa}        & 60.37          & 62.12           & 88.47           & 89.5           & 68.24           & 69.41          \\ \hline
	\textbf{Train}       & 78.52          & 80.05           & 88.7            & 90.43          & 88.52           & 88.52          \\ \hline
	\textbf{Tvmonitor}   & 79.23          & 79.34           & 92.8            & 92.93          & 85.38           & 85.38          \\ \hline
	\textbf{Mean Value}  & \textbf{70.5}  & \textbf{71.76}  & \textbf{88.65}  & \textbf{89.63} & \textbf{78.83}  & \textbf{79.33} \\ \hline
\end{tabular}
	}
	\vspace{-0.2cm}
	\caption{\label{tbl:pascal_detailed}{\bf Pascal VOC dataset.} Detailed class-wise panoptic segmentation results on the Pascal VOC validation set comparing results without BCRF vs with BCRF on a standard network.}
	\vspace{-0.5cm}
\end{table*}


